Learning to Correct 3D Reconstructions from Multiple Views

This paper is about reducing the cost of building good large-scale 3D reconstructions post-hoc. We render 2D views of an existing reconstruction and train a convolutional neural network (CNN) that refines inverse-depth to match a higher-quality reconstruction. Since the views that we correct are rendered from the same reconstruction, they share the same geometry, so overlapping views complement each other. We take advantage of that in two ways. Firstly, we impose a loss during training which guides predictions on neighbouring views to have the same geometry and has been shown to improve performance. Secondly, in contrast to previous work, which corrects each view independently, we also make predictions on sets of neighbouring views jointly. This is achieved by warping feature maps between views and thus bypassing memory-intensive 3D computation. We make the observation that features in the feature maps are viewpoint-dependent, and propose a method for transforming features with dynamic filters generated by a multi-layer perceptron from the relative poses between views. In our experiments we show that this last step is necessary for successfully fusing feature maps between views.

==> figures/feature-aggregation.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{figures/graphics/feature-aggregation.pdf}
\caption{
Feature map aggregation.
In the left column we show feature maps for a front view and a top view, along with inverse-depth images as reference.
To aggregate the top view with the front view, we first warp the top feature map into the front view.
The relative transform between the top and the front view, $\transform{front}{top}$, is used to generate the weights for a $1\times{}1$ convolution that transforms the \emph{features} from the top view to the front view.
Finally, the resulting feature map can be aggregated with the front view feature map.
Note that in the front feature map the features fade from green to violet towards the horizon, while in the warping of the top view, the features do not change with depth.
Only after transforming the \emph{features} do we see them fading towards the horizon.
For visualisation, the above feature maps are projected to three channels using the same random projection.
}
\label{fig:feature-aggregation}
\end{figure*}

==> figures/gross-errors.tex <==
\begin{figure}[t!]
\centering
\includegraphics{figures/graphics/gross-errors.eps}
\caption{%
Gross error correction.
For each threshold (Equation~\ref{eq:thresholded_accuracy}), we count how many pixels are incorrect in the predictions over the test set.
% Our full model removes 45.3\% of the smaller errors and 77.5\% of the gross errors.
% The baseline model is unable to effectively handle the multi-view setup, and fails to correct gross errors.
}
\label{fig:gross-errors}
\end{figure}

==> sections/5_discussion.tex <==
\section{Discussion}
\label{sec:discussion}


==> tables/hyperparameters.tex <==
\begin{table}
\caption{Summary of Hyperparameters Used in System}
\label{tab:hyperparameters}
\begin{tabular}{llp{5cm}}
\toprule
\textbf{Symbol}         & \textbf{Value}                & \textbf{Description} \\
\midrule
% $\epsilon$              & $10^{-4}$           & Minimum value for corrected inverse depth. \\
% $\scaling{\dataname}$   & 1                   & Weight of the data loss. \\
% $\scaling{\gradname}$   & 0.1                 & Weight of the smoothness loss. \\
% $\scaling{\gcname}$     & 0.1                 & Weight of the geometric consistency loss. \\
% $\scaling{\regname}$    & $10^{-6}$           & Weight of the $L_2$ variable regulariser. \\
% $w_{min}$                 & 0.1               & Minimum per-pixel loss scaling. \\
% $w_{max}$                 & 5                 & Maximum per-pixel loss scaling. \\
% \midrule
$\eta_{max}$ & $10^{-4}$ & Initial learning rate. \\
$\eta_{min}$ & $5\cdot10^{-6}$ & Final learning rate. \\
$T_{max}$ & $1.2\cdot10^5$ & Learning rate decay steps. \\
$\beta_1$ & 0.9 & Adam exponential decay rate for first moment estimates. \\
$\beta_2$ & 0.999 & Adam exponential decay rate for second moment estimates. \\
 & 80 & Norm at witch gradients are clipped during training. \\
 & 16 & Batch size. \\
 & $5\cdot10^5$ & Number of training steps. \\
\bottomrule
\end{tabular}
\end{table}
